Faster and Better LLMs via Latency-Aware Test-Time Scaling

Test-Time Scaling (TTS) has proven effective in improving the performance of Large Language Models (LLMs) during inference. However, existing research has overlooked the efficiency of TTS from a latency-sensitive perspective. Through a latency-aware evaluation of representative TTS methods, we demonstrate that a compute-optimal TTS does not always result in the lowest latency in scenarios where latency is critical. To address this gap and achieve latency-optimal TTS, we propose two key approaches by optimizing the concurrency configurations: (1) branch-wise parallelism, which leverages multiple concurrent inference branches, and (2) sequence-wise parallelism, enabled by speculative decoding. By integrating these two approaches and allocating computational resources properly to each, our latency-optimal TTS enables a 32B model to reach 82.3% accuracy on MATH-500 within 1 minute and a smaller 3B model to achieve 72.4% within 10 seconds. Our work emphasizes the importance of latency-aware TTS and demonstrates its ability to deliver both speed and accuracy in latency-sensitive scenarios.

==> sec/temp_outlines.tex <==
\textbf{Outlines of this paper: existing}
\\ 1 Introduction
\\ 2 Background
\\ \indent Test-time scaling
\\ \indent Measuring the budget of scaling 
\\ 3 Rethinking Test-Time Scaling with Latency
\\ \indent 3.1 Test-Time Scaling Should Consider Device-Side Latency
\\ \indent 3.2 Latency-Optimal Test-Time Scaling
\\ 4 How to Latency-Optimally Scale?
\\ \indent 4.1 Experiment setup
\\ \indent 4.2 How does TTS influence model latency
\\ \indent\indent Sequential scaling suffer from low throughput
\\ \indent\indent Parallel scaling scales fast, but limited
\\ \indent\indent Mostly, parallel scaling can surpass sequential scaling within limited time period.
\\ \indent 4.3 How do branches influence TTS w.r.t. latency
\\ \indent 4.4 How does speculative decoding influence TTS w.r.t latency
\\ 5 Results under Latency-Optimal TTS
\\ \indent 5.1 Can LLM solve the problem in 1 minutes?
\\ \indent 5.2 How can latency-optimal improve compared with baseline?
\\ 6 Conclusion

\newpage

\textbf{Outlines of this paper: new version}
\\ 1 Introduction
\\ 2 Background
\\ \indent Test-time scaling
\\ \indent \sout{Measuring the budget of scaling} 
\\ \indent \zhangm{Measurement of Scaling Budget} \zilim{\checkmark}
\\ 3 Rethinking Test-Time Scaling with Latency
\\ \indent \sout{3.1 Test-Time Scaling Should Consider Device-Side Latency}
\\ \indent \zhangm{3.1 Test-Time Scaling with Latency Budget} \zilim{\checkmark}
\\ \indent\indent  \zhangm{Token Efficiency}
\\ \indent\indent  \zhangm{Throughput}
\\ \indent \sout{3.2 Latency-Optimal Test-Time Scaling}
\\ \sout{4 How to Latency-Optimally Scale?}
\\ \indent \zhangm{3.2 How to Improve TTS with Latency Budget?} \zilim{\checkmark}
\\ \indent\indent  \zhangm{Branch-wise Parallelism}
\\ \indent\indent  \zhangm{Sequence-wise Parallelism}
\\ \indent\indent  \zhangm{The figure containing (red,green,+sd,+paral) should be placed here. This part is logically connected to the (B,gamma) in 3.3 equation}
\\ \indent \zhangm{3.3 Latency-Optimal Test-Time Scaling}
\\ \zhangm{4 Experiments and Discussion} \zilim{\checkmark}
\\ \indent 4.1 Experimental Setup
\\ \indent \sout{4.2 How does TTS influence model latency}
\\ \indent\indent \sout{Sequential scaling suffer from low throughput}
\\ \indent\indent \sout{Parallel scaling scales fast, but limited}
\\ \indent\indent \sout{Mostly, parallel scaling can surpass sequential scaling within limited time period.}
\\ \indent \zhangm{4.2 Parallel and Sequential Scaling under TTS with Latency Budget}
\\ \indent \sout{4.3 How do branches influence TTS w.r.t. latency} \zhangm{4.3 The Impact of Branch-wise Parallelism for TTS with Latency Budget}
\\ \indent \sout{4.4 How does speculative decoding influence TTS w.r.t latency} \zhangm{4.4 The Impact of Sequence-wise Parallelism for TTS with Latency Budget}
\\ \indent \zhangm{4.5 Achieving Latency-Optimal TTS with Branch-wise and Sequence-wise Parallelism}
\\ 5 Results under Latency-Optimal TTS
\\ \indent 5.1 Can LLM solve the problem in 1 minutes?
\\ \indent 5.2 How can latency-optimal improve compared with baseline?
\\ 6 Conclusion
\\ \zhangm{Limitation} \zilim{\checkmark}










